Using Zero-shot Prompting in the Automatic Creation and Expansion of Topic Taxonomies for Tagging Retail Banking Transactions

This work presents an unsupervised method for automatically constructing and expanding topic taxonomies using instruction-based fine-tuned LLMs (Large Language Models). We apply topic modeling and keyword extraction techniques to create initial topic taxonomies and LLMs to post-process the resulting terms and create a hierarchy. To expand an existing taxonomy with new terms, we use zero-shot prompting to find out where to add new nodes, which, to our knowledge, is the first work to present such an approach to taxonomy tasks. We use the resulting taxonomies to assign tags that characterize merchants from a retail bank dataset. To evaluate our work, we asked 12 volunteers to answer a two-part form in which we first assessed the quality of the taxonomies created and then the tags assigned to merchants based on that taxonomy. The evaluation revealed a coherence rate exceeding 90% for the chosen taxonomies. The taxonomies' expansion with LLMs also showed exciting results for parent node prediction, with an f1-score above 70% in our taxonomies.

==> chapters/3_background.tex <==
\section{Background}
%In this section, we provide a comprehensive background on Language Models (LMs), Large Language Models (LLMs), and the concept of Prompt-tuning. These concepts are essential to understanding the construction and editing of taxonomies utilizing LLMs.
In this section, we provide a comprehensive background on Large Language Models (LLMs), and the concept of Prompt-tuning. These concepts are essential to understanding the construction and editing of taxonomies utilizing LLMs.

%\subsection{Language Models}
%X - Language Models are computational models designed to understand and generate human language. They capture natural language's statistical patterns and structures, enabling machines to process, generate, and evaluate text. Recently, LMs have been studied in the field of NLP and have undergone significant advancements \cite{vaswani2017attention}.

%The main objective of LMs is to capture the probability distribution over sequences of words or tokens in a given language. By learning the co-occurrence patterns and dependencies between words, LMs can generate coherent and contextually appropriate text. 

%X - Recent breakthroughs in deep learning, particularly with the advent of Transformer models, have revolutionized the field of LMs \cite{vaswani2017attention}. Transformers employ self-attention mechanisms that allow for efficient modeling of long-range dependencies. Pre-trained LMs, such as OpenAI's GPT \cite{radford2019language} and Google's BERT \cite{devlin2018bert}, have achieved remarkable performance across a wide range of NLP tasks, including language generation, sentiment analysis, and named entity recognition.

%X - The versatility of LMs has led to their extensive adoption in various NLP applications. One prominent application is language generation, where LMs produce coherent and contextually relevant text. This includes automated summarization, dialogue generation, machine translation, and content creation.

%LMs have also proven invaluable in improving search engines, information retrieval systems, and recommendation algorithms by enhancing the understanding of user queries and document relevance. Furthermore, LMs have played a crucial role in improving language understanding tasks. Sentiment analysis, question-answering systems, named entity recognition, and part-of-speech tagging all benefit from the context-aware representations learned by LMs \cite{devlin2018bert}. 

%Additionally, methods like few-shot learning and prompt engineering have been proposed to enhance the fine-tuning process and enable more efficient adaptation to specific tasks and domains \cite{liu2019roberta}.

\subsection{Large Language Models}
Lately, Large Language Models (LLMs) have garnered significant attention for their exceptional performance in various NLP tasks. LLMs, such as GPT-3 \cite{brown2020language} and LLAMA \cite{touvron2023llama}, are characterized by their massive scale, comprising billions of parameters and being trained on vast data. LLMs are often pre-trained in an unsupervised manner on a large corpus of text, such as books, articles, and web pages, allowing them to learn contextual representations that capture the intricacies of human language.

To use LLMs for specific purposes, a highly effective approach is to fine-tune them on task-specific data. Fine-tuning enables LLMs to adapt to specific domains or tasks with minimal labeled data, significantly reducing the need for large annotated datasets. InstructGPT proposes a method called RLHF (Reinforcement Learning from Human Feedback), which involves fine-tuning large models using PPO (Proximal Policy Optimization) based on a reward model trained to align the models with human preferences~\cite{ouyang2022training}. In our method and experiments, we used ChatGPT, a sibling model to InstructGPT ~\cite{openai2023gpt4}. %The flexibility of LLMs makes them valuable in scenarios where labeled data is scarce or difficult to obtain \cite{raffel2020exploring}.

%InstructGPT proposes a method called RLHF (Reinforcement Learning from Human Feedback), which involves fine-tuning large models using PPO (Proximal Policy Optimization) based on a reward model trained to align the models with human preferences~\cite{ouyang2022training}. This approach is also employed by ChatGPT. The reward model is trained using comparison data generated by human labelers who rank the model outputs manually. Based on these rankings, the reward model or a machine labeler calculates a reward that is then utilized to update the FM through PPO.

%A notable advancement in FM technology is GPT-4~\cite{openai2023gpt4}. GPT-4 employs a pre-training phase where it predicts the next token in a document, followed by RLHF fine-tuning. GPT-4 surpasses GPT-3.5 in terms of reliability, creativity, and ability to handle more detailed instructions as the complexity of the task increases.

%This approach is also employed by ChatGPT, based on GPT-4~\cite{openai2023gpt4}. GPT-4 employs a pre-training phase where it predicts the next token in a document, followed by RLHF fine-tuning. GPT-4 surpasses GPT-3.5 in terms of reliability, creativity, and ability to handle more detailed instructions as the complexity of the task increases.


%To use LLMs for specific purposes, a highly effective approach is to fine-tune them on task-specific data. Fine-tuning enables LLMs to adapt to specific domains or tasks with minimal labeled data, significantly reducing the need for large annotated datasets. The flexibility of LLMs makes them valuable in scenarios where labeled data is scarce or difficult to obtain \cite{raffel2020exploring}.
%Transfer learning, a technique where LLMs are fine-tuned on task-specific data, has proven to be a highly effective approach. Fine-tuning enables LLMs to adapt to specific domains or tasks with minimal labeled data, significantly reducing the need for large annotated datasets. The flexibility of LLMs makes them valuable in scenarios where labeled data is scarce or difficult to obtain \cite{raffel2020exploring}.

%However, the use of LLMs also raises concerns regarding ethical considerations, biases, and data privacy. Given the scale of these models and the data they are trained on, biases in the training data can manifest in the generated text. Researchers have been actively exploring methods to mitigate biases and ensure fairness in LLMs \cite{bolukbasi2016man}. Additionally, privacy concerns arise due to the potential of inadvertently memorizing and revealing sensitive information during fine-tuning or text generation \cite{carlini2019secret}.

\subsection{Prompt Tuning}
%Prompt-tuning and Fine-tuning are two critical techniques used to enhance the performance and adaptability of Large Language Models (LLMs) in specific tasks or domains. These approaches allow researchers and practitioners to tailor the behavior and output of LLMs, making them more suitable for targeted applications.

%Prompt-tuning involves the design and optimization of prompts or instruction formats for LLMs \cite{brown2020language}. By leveraging prompt engineering, researchers can improve the control and precision of LLM outputs. Techniques such as template-based prompts, rule-based prompts, and cloze-style prompts have been explored to guide LLMs toward desired responses. The effectiveness of prompt tuning has been demonstrated in various applications, including question-answering, summarization, and dialogue generation.

Prompt-tuning and Fine-tuning are two critical techniques used to enhance the performance and adaptability of Large Language Models (LLMs) in specific tasks or domains. These approaches allow researchers and practitioners to tailor the behavior and output of LLMs, making them more suitable for targeted applications.

Prompt-tuning involves the design and optimization of prompts or instruction formats for LLMs \cite{brown2020language}. By leveraging prompt engineering, researchers can improve the control and precision of LLM outputs. Fine-tuning complements prompt tuning by adapting pre-trained LLMs to specific tasks or domains. After pre-training on a large corpus of general text data, LLMs are fine-tuned on smaller task-specific datasets with labeled examples. This process allows LLMs to learn task-specific nuances, capturing domain-specific features, which can improve the LLM performance on the target task.


%The choice of prompt greatly influences the generated output, and by carefully crafting prompts, researchers can guide the model's responses toward desired behaviors. For example, in language translation, a prompt can specify the source language and desired target language to ensure accurate and fluent translations.

%Fine-tuning complements prompt tuning by adapting pre-trained LLMs to specific tasks or domains. After pre-training on a large corpus of general text data, LLMs are fine-tuned on smaller task-specific datasets with labeled examples. This process allows LLMs to learn task-specific nuances, capturing domain-specific features, which can improve the LLM performance on the target task.



